Area law for three-dimensional U(1) lattice gauge theory with the Wilson action at every coupling

We prove that three-dimensional U(1) lattice gauge theory with the Wilson action confines static charges at every coupling: rectangular Wilson loops obey an area law, uniformly in the finite box, with an explicit lower bound on the string tension at weak coupling. For the Villain action, confinement at every coupling is the theorem of G\"opfert and Mack; for the Wilson action the question had remained open. The Wilson weight is a mixture of Villain weights, so Ginibre's inequality bounds the Wilson loop by an average of Villain loops at a coupling larger by a fixed factor, in which a sparse random set of plaquettes is frozen at angle zero; after this set is regularized, the multiscale analysis of G\"opfert and Mack, made uniform in it, and a Peierls estimate give the area law. As corollaries, the area law holds at every coupling for all closed subgroups of U(n) containing the scalars, also with a Higgs field blind to the centre of U(n), and for the Georgi--Glashow model at infinite Higgs coupling.

==> s4labels.tex <==
% s4labels.tex: the \newlabel lines of Part S4's s4.aux (version 4 build) with the prefix S4-, as xr's
% \externaldocument[S4-]{s4} would read them; arXiv deletes .aux files.
\makeatletter
\newlabel{S4-S:S4.0}{{S4.0}{3}{}{section.0}{}}
\newlabel{S4-S:S4.1}{{S4.1}{4}{}{section.1}{}}
\newlabel{S4-B1-s:grid}{{S4.1.1}{4}{}{subsection.1.1}{}}
\newlabel{S4-B1-def:grid1d}{{S4.1.1}{4}{}{theorem.1.1}{}}
\newlabel{S4-B1-lem:1d}{{S4.1.2}{5}{}{theorem.1.2}{}}
\newlabel{S4-B1-lem:33}{{S4.1.3}{6}{}{theorem.1.3}{}}
\newlabel{S4-B1-lem:G15}{{S4.1.4}{6}{}{theorem.1.4}{}}
\newlabel{S4-B1-rem:marks}{{S4.1.5}{6}{}{theorem.1.5}{}}
\newlabel{S4-B1-s:align}{{S4.1.2}{6}{}{subsection.1.2}{}}
\newlabel{S4-B1-lem:35}{{S4.1.6}{6}{}{theorem.1.6}{}}
\newlabel{S4-B1-s:minimizers}{{S4.1.3}{7}{}{subsection.1.3}{}}
\newlabel{S4-B1-lem:latmin}{{S4.1.8}{7}{}{theorem.1.8}{}}
\newlabel{S4-B1-lem:39}{{S4.1.9}{7}{}{theorem.1.9}{}}
\newlabel{S4-B1-lem:312}{{S4.1.10}{8}{}{theorem.1.10}{}}
\newlabel{S4-B1-s:history}{{S4.1.4}{8}{}{subsection.1.4}{}}
\newlabel{S4-B1-def:hist}{{S4.1.12}{8}{}{theorem.1.12}{}}
\newlabel{S4-B1-lem:42}{{S4.1.13}{9}{}{theorem.1.13}{}}
\newlabel{S4-B1-rem:phase1Sbar}{{S4.1.14}{9}{}{theorem.1.14}{}}
\newlabel{S4-B1-prop:43}{{S4.1.15}{10}{}{theorem.1.15}{}}
\newlabel{S4-B1-ss:aux}{{S4.1.4.1}{11}{}{subsubsection.1.4.1}{}}
\newlabel{S4-B1-def:aux}{{S4.1.16}{11}{}{theorem.1.16}{}}
\newlabel{S4-B1-lem:414}{{S4.1.17}{11}{}{theorem.1.17}{}}
\newlabel{S4-B1-lem:ph1term}{{S4.1.18}{12}{}{theorem.1.18}{}}
\newlabel{S4-B1-s:segments}{{S4.1.5}{12}{}{subsection.1.5}{}}
\newlabel{S4-B1-def:segments}{{S4.1.19}{12}{}{theorem.1.19}{}}
\newlabel{S4-B1-lem:segid}{{S4.1.20}{13}{}{theorem.1.20}{}}
\newlabel{S4-B1-lem:46}{{S4.1.21}{14}{}{theorem.1.21}{}}
\newlabel{S4-B1-rem:cor410}{{S4.1.22}{14}{}{theorem.1.22}{}}
\newlabel{S4-B1-lem:48}{{S4.1.23}{14}{}{theorem.1.23}{}}
\newlabel{S4-B1-s:runs}{{S4.1.6}{15}{}{subsection.1.6}{}}
\newlabel{S4-B1-def:thin}{{S4.1.24}{15}{}{theorem.1.24}{}}
\newlabel{S4-B1-lem:runs}{{S4.1.25}{15}{}{theorem.1.25}{}}
\newlabel{S4-B1-lem:linesides}{{S4.1.26}{16}{}{theorem.1.26}{}}
\newlabel{S4-B1-lem:thin}{{S4.1.27}{16}{}{theorem.1.27}{}}
\newlabel{S4-B1-prop:415}{{S4.1.28}{17}{}{theorem.1.28}{}}
\newlabel{S4-B1-s:rest}{{S4.1.7}{17}{}{subsection.1.7}{}}
\newlabel{S4-B1-thm:416c}{{S4.1.29}{17}{}{theorem.1.29}{}}
\newlabel{S4-B1-s:ucells}{{S4.1.8}{18}{}{subsection.1.8}{}}
\newlabel{S4-B1-lem:421}{{S4.1.30}{18}{}{theorem.1.30}{}}
\newlabel{S4-B1-rem:421app}{{S4.1.31}{19}{}{theorem.1.31}{}}
\newlabel{S4-B1-s:cutorder}{{S4.1.9}{19}{}{subsection.1.9}{}}
\newlabel{S4-B1-def:cutorder}{{S4.1.32}{19}{}{theorem.1.32}{}}
\newlabel{S4-B1-prop:anyorder}{{S4.1.33}{19}{}{theorem.1.33}{}}
\newlabel{S4-B1-rem:cutuses}{{S4.1.34}{20}{}{theorem.1.34}{}}
\newlabel{S4-B1-s:finecoarse}{{S4.1.10}{20}{}{subsection.1.10}{}}
\newlabel{S4-B1-def:fine}{{S4.1.35}{20}{}{theorem.1.35}{}}
\newlabel{S4-B1-lem:blowup}{{S4.1.36}{20}{}{theorem.1.36}{}}
\newlabel{S4-B1-lem:419coarse}{{S4.1.37}{20}{}{theorem.1.37}{}}
\newlabel{S4-B1-lem:419fine}{{S4.1.38}{21}{}{theorem.1.38}{}}
\newlabel{S4-B1-lem:finer}{{S4.1.39}{21}{}{theorem.1.39}{}}
\newlabel{S4-B1-s:cs}{{S4.1.11}{22}{}{subsection.1.11}{}}
\newlabel{S4-B1-s:cheeger}{{S4.1.12}{22}{}{subsection.1.12}{}}
\newlabel{S4-B1-lem:cheeger}{{S4.1.40}{22}{}{theorem.1.40}{}}
\newlabel{S4-B1-lem:418}{{S4.1.41}{22}{}{theorem.1.41}{}}
\newlabel{S4-B1-lem:ball}{{S4.1.42}{22}{}{theorem.1.42}{}}
\newlabel{S4-S:S4.2}{{S4.2}{23}{}{section.2}{}}
\newlabel{S4-C5-s:topology}{{S4.2.1}{23}{}{subsection.2.1}{}}
\newlabel{S4-C5-lem:acyclic}{{S4.2.1}{23}{}{theorem.2.1}{}}
\newlabel{S4-C5-lem:sphere}{{S4.2.2}{23}{}{theorem.2.2}{}}
\newlabel{S4-C5-lem:timar}{{S4.2.3}{24}{}{theorem.2.3}{}}
\newlabel{S4-C5-s:51}{{S4.2.2}{24}{}{subsection.2.2}{}}
\newlabel{S4-C5-thm:51}{{S4.2.4}{24}{}{theorem.2.4}{}}
\newlabel{S4-C5-eq:51}{{{5.1}}{24}{}{theorem.2.4}{}}
\newlabel{S4-C5-eq:52}{{{5.2}}{24}{}{equation.2.1}{}}
\newlabel{S4-C5-eq:etaorder}{{{$\eta _{T}$}}{25}{}{equation.2.1}{}}
\newlabel{S4-C5-s:52}{{S4.2.3}{25}{}{subsection.2.3}{}}
\newlabel{S4-C5-lem:52}{{S4.2.5}{25}{}{theorem.2.5}{}}
\newlabel{S4-C5-lem:53disp}{{S4.2.6}{26}{}{theorem.2.6}{}}
\newlabel{S4-C5-eq:53}{{{5.3}}{26}{}{equation.2.1}{}}
\newlabel{S4-C5-lem:54}{{S4.2.7}{26}{}{theorem.2.7}{}}
\newlabel{S4-C5-eq:54}{{{5.4}}{26}{}{equation.2.1}{}}
\newlabel{S4-C5-lem:55}{{S4.2.8}{26}{}{theorem.2.8}{}}
\newlabel{S4-C5-prop:55}{{S4.2.9}{27}{}{theorem.2.9}{}}
\newlabel{S4-C5-eq:55}{{{5.5}}{27}{}{equation.2.1}{}}
\newlabel{S4-C5-s:53}{{S4.2.4}{27}{}{subsection.2.4}{}}
\newlabel{S4-C5-lem:56}{{S4.2.10}{27}{}{theorem.2.10}{}}
\newlabel{S4-C5-lem:57}{{S4.2.11}{27}{}{theorem.2.11}{}}
\newlabel{S4-C5-lem:58}{{S4.2.12}{28}{}{theorem.2.12}{}}
\newlabel{S4-C5-eq:epsc}{{{$\varepsilon _{c}$}}{28}{}{equation.2.1}{}}
\newlabel{S4-C5-prop:59}{{S4.2.13}{28}{}{theorem.2.13}{}}
\newlabel{S4-C5-lem:510}{{S4.2.14}{29}{}{theorem.2.14}{}}
\newlabel{S4-C5-prop:511}{{S4.2.15}{29}{}{theorem.2.15}{}}
\newlabel{S4-C5-lem:512}{{S4.2.16}{30}{}{theorem.2.16}{}}
\newlabel{S4-C5-eq:56}{{{5.6}}{30}{}{equation.2.1}{}}
\newlabel{S4-C5-s:54}{{S4.2.5}{30}{}{subsection.2.5}{}}
\newlabel{S4-C5-def:513}{{S4.2.17}{31}{}{theorem.2.17}{}}
\newlabel{S4-C5-lem:514}{{S4.2.18}{31}{}{theorem.2.18}{}}
\newlabel{S4-C5-lem:cheeger}{{S4.2.19}{32}{}{theorem.2.19}{}}
\newlabel{S4-C5-lem:annulus}{{S4.2.20}{33}{}{theorem.2.20}{}}
\newlabel{S4-C5-lem:shellclaim}{{S4.2.21}{33}{}{theorem.2.21}{}}
\newlabel{S4-C5-lem:515}{{S4.2.22}{33}{}{theorem.2.22}{}}
\newlabel{S4-C5-lem:516}{{S4.2.23}{34}{}{theorem.2.23}{}}
\newlabel{S4-C5-s:55}{{S4.2.6}{34}{}{subsection.2.6}{}}
\newlabel{S4-C5-lem:517}{{S4.2.24}{35}{}{theorem.2.24}{}}
\newlabel{S4-C5-eq:RNF}{{{$R_{\mathrm  {NF}}$}}{35}{}{equation.2.1}{}}
\newlabel{S4-C5-lem:518}{{S4.2.25}{36}{}{theorem.2.25}{}}
\newlabel{S4-C5-prop:519}{{S4.2.26}{37}{}{theorem.2.26}{}}
\newlabel{S4-C5-eq:57}{{{5.7}}{37}{}{equation.2.1}{}}
\newlabel{S4-C5-s:56}{{S4.2.7}{38}{}{subsection.2.7}{}}
\newlabel{S4-C5-lem:520}{{S4.2.27}{38}{}{theorem.2.27}{}}
\newlabel{S4-C5-lem:521}{{S4.2.28}{39}{}{theorem.2.28}{}}
\newlabel{S4-C5-eq:Cresp}{{{$C_{\mathrm  {resp}}$}}{40}{}{equation.2.1}{}}
\newlabel{S4-C5-s:57}{{S4.2.8}{40}{}{subsection.2.8}{}}
\newlabel{S4-C5-eq:58}{{{5.8}}{40}{}{equation.2.1}{}}
\newlabel{S4-C5-lem:walk}{{S4.2.29}{40}{}{theorem.2.29}{}}
\newlabel{S4-C5-prop:522}{{S4.2.30}{41}{}{theorem.2.30}{}}
\newlabel{S4-C5-eq:59}{{{5.9}}{42}{}{equation.2.1}{}}
\newlabel{S4-C5-lem:523}{{S4.2.31}{42}{}{theorem.2.31}{}}
\newlabel{S4-C5-prop:524}{{S4.2.32}{43}{}{theorem.2.32}{}}
\newlabel{S4-C5-lem:525}{{S4.2.33}{43}{}{theorem.2.33}{}}
\newlabel{S4-C5-lem:526}{{S4.2.34}{43}{}{theorem.2.34}{}}
\newlabel{S4-C5-ss:proof51}{{S4.2.8.1}{44}{}{subsubsection.2.8.1}{}}
\newlabel{S4-C5-eq:510}{{{5.10}}{44}{}{equation.2.1}{}}
\newlabel{S4-C5-ss:sharper}{{S4.2.8.2}{45}{}{subsubsection.2.8.2}{}}
\newlabel{S4-C5-lem:526A}{{S4.2.35}{45}{}{theorem.2.35}{}}
\newlabel{S4-C5-lem:526B}{{S4.2.36}{46}{}{theorem.2.36}{}}
\newlabel{S4-C5-cor:sharper}{{S4.2.37}{46}{}{theorem.2.37}{}}
\newlabel{S4-C5-rem:sharper}{{S4.2.38}{47}{}{theorem.2.38}{}}
\newlabel{S4-C5-s:constants}{{S4.2.9}{47}{}{subsection.2.9}{}}
\newlabel{S4-S:S4.3}{{S4.3}{49}{}{section.3}{}}
\newlabel{S4-C1-C1:sec:kernel}{{S4.3.1}{49}{}{subsection.3.1}{}}
\newlabel{S4-C1-C1:rem:thomson}{{S4.3.1}{49}{}{theorem.3.1}{}}
\newlabel{S4-C1-C1:ssec:Z3}{{S4.3.1.2}{49}{}{subsubsection.3.1.2}{}}
\newlabel{S4-C1-C1:def:vZ3}{{S4.3.3}{49}{}{theorem.3.3}{}}
\newlabel{S4-C1-C1:lem:Z3}{{S4.3.4}{49}{}{theorem.3.4}{}}
\newlabel{S4-C1-C1:rem:vcb}{{S4.3.5}{50}{}{theorem.3.5}{}}
\newlabel{S4-C1-C1:sec:rep}{{S4.3.2}{50}{}{subsection.3.2}{}}
\newlabel{S4-C1-C1:lem:poisson}{{S4.3.6}{50}{}{theorem.3.6}{}}
\newlabel{S4-C1-C1:rem:Zpos}{{S4.3.7}{51}{}{theorem.3.7}{}}
\newlabel{S4-C1-C1:sec:mayer}{{S4.3.3}{52}{}{subsection.3.3}{}}
\newlabel{S4-C1-C1:ssec:setting}{{S4.3.3.1}{52}{}{subsubsection.3.3.1}{}}
\newlabel{S4-C1-C1:eq:H1}{{S4.3.1}{52}{}{equation.3.1}{}}
\newlabel{S4-C1-C1:def:vertex}{{S4.3.8}{52}{}{theorem.3.8}{}}
\newlabel{S4-C1-C1:eq:vertex}{{S4.3.2}{52}{}{equation.3.2}{}}
\newlabel{S4-C1-C1:lem:local}{{S4.3.9}{52}{}{theorem.3.9}{}}
\newlabel{S4-C1-C1:ssec:boltz}{{S4.3.3.2}{53}{}{subsubsection.3.3.2}{}}
\newlabel{S4-C1-C1:prop:boltz}{{S4.3.10}{53}{}{theorem.3.10}{}}
\newlabel{S4-C1-C1:eq:boltz}{{S4.3.3}{53}{}{equation.3.3}{}}
\newlabel{S4-C1-C1:prop:exp}{{S4.3.11}{54}{}{theorem.3.11}{}}
\newlabel{S4-C1-C1:eq:expform}{{S4.3.4}{54}{}{equation.3.4}{}}
\newlabel{S4-C1-C1:rem:yukawa}{{S4.3.12}{54}{}{theorem.3.12}{}}
\newlabel{S4-C1-C1:prop:coef}{{S4.3.13}{54}{}{theorem.3.13}{}}
\newlabel{S4-C1-C1:eq:rho}{{S4.3.5}{54}{}{equation.3.5}{}}
\newlabel{S4-C1-C1:lem:intrinsic}{{S4.3.14}{55}{}{theorem.3.14}{}}
\newlabel{S4-C1-C1:sec:stab}{{S4.3.4}{55}{}{subsection.3.4}{}}
\newlabel{S4-C1-C1:def:split}{{S4.3.15}{55}{}{theorem.3.15}{}}
\newlabel{S4-C1-C1:def:stab}{{S4.3.16}{55}{}{theorem.3.16}{}}
\newlabel{S4-C1-C1:eq:stab}{{S4.3.6}{55}{}{equation.3.6}{}}
\newlabel{S4-C1-C1:eq:E1}{{S4.3.7}{56}{}{equation.3.7}{}}
\newlabel{S4-C1-C1:prop:GM8}{{S4.3.17}{56}{}{theorem.3.17}{}}
\newlabel{S4-C1-C1:prop:64}{{S4.3.19}{56}{}{theorem.3.19}{}}
\newlabel{S4-C1-C1:sec:est}{{S4.3.5}{57}{}{subsection.3.5}{}}
\newlabel{S4-C1-C1:ssec:trees}{{S4.3.5.1}{57}{}{subsubsection.3.5.1}{}}
\newlabel{S4-C1-C1:lem:bkar}{{S4.3.20}{57}{}{theorem.3.20}{}}
\newlabel{S4-C1-C1:cor:tree}{{S4.3.21}{57}{}{theorem.3.21}{}}
\newlabel{S4-C1-C1:lem:decouple}{{S4.3.22}{58}{}{theorem.3.22}{}}
\newlabel{S4-C1-C1:lem:treebound}{{S4.3.23}{58}{}{theorem.3.23}{}}
\newlabel{S4-C1-C1:eq:utree}{{S4.3.8}{58}{}{equation.3.8}{}}
\newlabel{S4-C1-C1:eq:ubound}{{S4.3.9}{58}{}{equation.3.9}{}}
\newlabel{S4-C1-C1:lem:cayley}{{S4.3.24}{58}{}{theorem.3.24}{}}
\newlabel{S4-C1-C1:ssec:norms}{{S4.3.5.2}{58}{}{subsubsection.3.5.2}{}}
\newlabel{S4-C1-C1:lem:GM6}{{S4.3.25}{58}{}{theorem.3.25}{}}
\newlabel{S4-C1-C1:def:norms}{{S4.3.26}{59}{}{theorem.3.26}{}}
\newlabel{S4-C1-C1:prop:onestep}{{S4.3.27}{59}{}{theorem.3.27}{}}
\newlabel{S4-C1-C1:cor:iter}{{S4.3.29}{60}{}{theorem.3.29}{}}
\newlabel{S4-C1-C1:ssec:level1}{{S4.3.5.3}{60}{}{subsubsection.3.5.3}{}}
\newlabel{S4-C1-C1:lem:level1}{{S4.3.30}{60}{}{theorem.3.30}{}}
\newlabel{S4-C1-C1:ssec:link}{{S4.3.5.4}{60}{}{subsubsection.3.5.4}{}}
\newlabel{S4-C1-C1:lem:425}{{S4.3.31}{61}{}{theorem.3.31}{}}
\newlabel{S4-C1-C1:def:debye}{{S4.3.32}{61}{}{theorem.3.32}{}}
\newlabel{S4-C1-C1:lem:hyp}{{S4.3.33}{61}{}{theorem.3.33}{}}
\newlabel{S4-C1-C1:rem:debye}{{S4.3.34}{61}{}{theorem.3.34}{}}
\newlabel{S4-C1-C1:ssec:prop9}{{S4.3.5.5}{61}{}{subsubsection.3.5.5}{}}
\newlabel{S4-C1-C1:prop:9}{{S4.3.35}{61}{}{theorem.3.35}{}}
\newlabel{S4-C1-C1:thm:65}{{S4.3.36}{61}{}{theorem.3.36}{}}
\newlabel{S4-C1-C1:eq:lead}{{{6.7}}{62}{}{equation.3.10}{}}
\newlabel{S4-C1-C1:cor:S2plus}{{S4.3.37}{63}{}{theorem.3.37}{}}
\newlabel{S4-C1-C1:ssec:ref}{{S4.3.5.6}{64}{}{subsubsection.3.5.6}{}}
\newlabel{S4-C1-C1:def:ref}{{S4.3.39}{64}{}{theorem.3.39}{}}
\newlabel{S4-C1-C1:rem:refdef}{{S4.3.40}{64}{}{theorem.3.40}{}}
\newlabel{S4-C1-C1:prop:S4ref}{{S4.3.41}{64}{}{theorem.3.41}{}}
\newlabel{S4-C1-C1:prop:66}{{S4.3.42}{66}{}{theorem.3.42}{}}
\newlabel{S4-C1-C1:ssec:mass}{{S4.3.5.7}{66}{}{subsubsection.3.5.7}{}}
\newlabel{S4-C1-C1:prop:mass}{{S4.3.43}{66}{}{theorem.3.43}{}}
\newlabel{S4-C1-C1:eq:massfp}{{{6.11}}{66}{}{equation.3.10}{}}
\newlabel{S4-C1-C1:cor:S4debye}{{S4.3.45}{67}{}{theorem.3.45}{}}
\newlabel{S4-C1-C1:rem:S4uses}{{S4.3.46}{67}{}{theorem.3.46}{}}
\newlabel{S4-C1-C1:sec:ctf}{{S4.3.6}{67}{}{subsection.3.6}{}}
\newlabel{S4-C1-C1:lem:box}{{S4.3.47}{68}{}{theorem.3.47}{}}
\newlabel{S4-C1-C1:lem:face}{{S4.3.48}{68}{}{theorem.3.48}{}}
\newlabel{S4-C1-C1:eq:diam}{{S4.3.10}{70}{}{equation.3.10}{}}
\newlabel{S4-C1-C1:sec:hk}{{S4.3.7}{70}{}{subsection.3.7}{}}
\newlabel{S4-C1-C1:eq:HK1}{{S4.3.11}{70}{}{equation.3.11}{}}
\newlabel{S4-C1-C1:lem:moment}{{S4.3.49}{70}{}{theorem.3.49}{}}
\newlabel{S4-C1-C1:lem:exit}{{S4.3.50}{71}{}{theorem.3.50}{}}
\newlabel{S4-C1-C1:lem:BB}{{S4.3.51}{71}{}{theorem.3.51}{}}
\newlabel{S4-C1-C1:sec:rest}{{S4.3.8}{72}{}{subsection.3.8}{}}
\newlabel{S4-C1-C1:lem:skellam}{{S4.3.55}{72}{}{theorem.3.55}{}}
\newlabel{S4-S:S4.4}{{S4.4}{74}{}{section.4}{}}
\newlabel{S4-C2b-B:sec:71}{{S4.4.1}{74}{}{subsection.4.1}{}}
\newlabel{S4-C2b-B:lem:ops}{{S4.4.1}{74}{}{theorem.4.1}{}}
\newlabel{S4-C2b-B:lem:72}{{S4.4.2}{74}{}{theorem.4.2}{}}
\newlabel{S4-C2b-B:eq:S4}{{S4.4.1}{74}{}{equation.4.1}{}}
\newlabel{S4-C2b-B:eq:G23}{{S4.4.2}{75}{}{equation.4.2}{}}
\newlabel{S4-C2b-B:prop:75}{{S4.4.3}{75}{}{theorem.4.3}{}}
\newlabel{S4-C2b-B:cor:75}{{S4.4.4}{76}{}{theorem.4.4}{}}
\newlabel{S4-C2b-B:lem:76}{{S4.4.6}{77}{}{theorem.4.6}{}}
\newlabel{S4-C2b-B:sec:72}{{S4.4.2}{78}{}{subsection.4.2}{}}
\newlabel{S4-C2b-B:def:72}{{S4.4.7}{78}{}{theorem.4.7}{}}
\newlabel{S4-C2b-B:prop:78}{{S4.4.8}{78}{}{theorem.4.8}{}}
\newlabel{S4-C2b-B:prop:79}{{S4.4.9}{79}{}{theorem.4.9}{}}
\newlabel{S4-C2b-B:cor:710}{{S4.4.10}{79}{}{theorem.4.10}{}}
\newlabel{S4-C2b-B:sec:73}{{S4.4.3}{80}{}{subsection.4.3}{}}
\newlabel{S4-C2b-B:lem:711}{{S4.4.11}{80}{}{theorem.4.11}{}}
\newlabel{S4-C2b-B:lem:712}{{S4.4.12}{81}{}{theorem.4.12}{}}
\newlabel{S4-C2b-B:thm:713}{{S4.4.13}{81}{}{theorem.4.13}{}}
\newlabel{S4-C2b-B:thm:714}{{S4.4.14}{82}{}{theorem.4.14}{}}
\newlabel{S4-C2b-B:sec:74}{{S4.4.4}{82}{}{subsection.4.4}{}}
\newlabel{S4-C2b-B:lem:pf}{{S4.4.15}{82}{}{theorem.4.15}{}}
\newlabel{S4-C2b-B:lem:715}{{S4.4.16}{82}{}{theorem.4.16}{}}
\newlabel{S4-C2b-B:thm:716}{{S4.4.17}{83}{}{theorem.4.17}{}}
\newlabel{S4-C2b-B:cor:717}{{S4.4.18}{83}{}{theorem.4.18}{}}
\newlabel{S4-C2b-B:cor:718}{{S4.4.19}{84}{}{theorem.4.19}{}}
\newlabel{S4-C2b-B:prop:719}{{S4.4.20}{84}{}{theorem.4.20}{}}
\newlabel{S4-C2b-B:sec:75}{{S4.4.5}{85}{}{subsection.4.5}{}}
\newlabel{S4-C2b-B:def:wf}{{S4.4.21}{85}{}{theorem.4.21}{}}
\newlabel{S4-C2b-B:lem:720}{{S4.4.22}{85}{}{theorem.4.22}{}}
\newlabel{S4-C2b-B:lem:723}{{S4.4.23}{86}{}{theorem.4.23}{}}
\newlabel{S4-C2b-B:lem:721}{{S4.4.24}{87}{}{theorem.4.24}{}}
\newlabel{S4-C2b-B:lem:724}{{S4.4.25}{87}{}{theorem.4.25}{}}
\newlabel{S4-C2b-B:def:725}{{S4.4.26}{88}{}{theorem.4.26}{}}
\newlabel{S4-C2b-B:lem:725}{{S4.4.27}{88}{}{theorem.4.27}{}}
\newlabel{S4-C2b-B:lem:bridge}{{S4.4.28}{89}{}{theorem.4.28}{}}
\newlabel{S4-C2b-B:rem:nobridge}{{S4.4.29}{89}{}{theorem.4.29}{}}
\newlabel{S4-C2b-B:lem:726}{{S4.4.30}{89}{}{theorem.4.30}{}}
\newlabel{S4-C2b-B:thm:727}{{S4.4.31}{90}{}{theorem.4.31}{}}
\newlabel{S4-C2b-B:cor:728}{{S4.4.32}{92}{}{theorem.4.32}{}}
\newlabel{S4-C2b-B:sec:appC}{{S4.4.6}{92}{}{subsection.4.6}{}}
\newlabel{S4-S:S4.5}{{S4.5}{93}{}{section.5}{}}
\newlabel{S4-C2-C2:sec:GM6}{{S4.5.1}{93}{}{subsection.5.1}{}}
\newlabel{S4-C2-C2:eq:Href}{{S4.5.1}{93}{}{equation.5.1}{}}
\newlabel{S4-C2-C2:eq:Veffk}{{S4.5.2}{93}{}{equation.5.2}{}}
\newlabel{S4-C2-C2:prop:73}{{S4.5.1}{93}{}{theorem.5.1}{}}
\newlabel{S4-C2-C2:eq:7S1}{{S4.5.3}{93}{}{equation.5.3}{}}
\newlabel{S4-C2-C2:eq:rOmega}{{S4.5.4}{94}{}{equation.5.4}{}}
\newlabel{S4-C2-C2:eq:G2}{{S4.5.5}{94}{}{equation.5.5}{}}
\newlabel{S4-C2-C2:prop:74}{{S4.5.2}{94}{}{theorem.5.2}{}}
\newlabel{S4-C2-C2:eq:GM612}{{S4.5.6}{94}{}{equation.5.6}{}}
\newlabel{S4-C2-C2:eq:peierls1}{{S4.5.7}{95}{}{equation.5.7}{}}
\newlabel{S4-C2-C2:rem:612}{{S4.5.3}{95}{}{theorem.5.3}{}}
\newlabel{S4-C2-C2:prop:78}{{S4.5.4}{96}{}{theorem.5.4}{}}
\newlabel{S4-C2-C2:eq:translated}{{S4.5.8}{96}{}{equation.5.8}{}}
\newlabel{S4-C2-C2:eq:Nconst}{{S4.5.9}{96}{}{equation.5.9}{}}
\newlabel{S4-C2-C2:eq:lebesgue}{{S4.5.10}{96}{}{equation.5.10}{}}
\newlabel{S4-C2-C2:rem:handoff}{{S4.5.5}{97}{}{theorem.5.5}{}}
\newlabel{S4-C2-C2:sec:gauss}{{S4.5.2}{97}{}{subsection.5.2}{}}
\newlabel{S4-C2-C2:lem:marg}{{S4.5.6}{97}{}{theorem.5.6}{}}
\newlabel{S4-C2-C2:lem:margin-equiv}{{S4.5.7}{97}{}{theorem.5.7}{}}
\newlabel{S4-C2-C2:def:classes}{{S4.5.8}{97}{}{theorem.5.8}{}}
\newlabel{S4-C2-C2:lem:dom}{{S4.5.9}{98}{}{theorem.5.9}{}}
\newlabel{S4-C2-C2:lem:ibp}{{S4.5.10}{98}{}{theorem.5.10}{}}
\newlabel{S4-C2-C2:eq:ibp}{{S4.5.11}{98}{}{equation.5.11}{}}
\newlabel{S4-C2-C2:def:interp}{{S4.5.12}{99}{}{theorem.5.12}{}}
\newlabel{S4-C2-C2:eq:pi}{{S4.5.12}{99}{}{equation.5.12}{}}
\newlabel{S4-C2-C2:rem:BF212}{{S4.5.13}{99}{}{theorem.5.13}{}}
\newlabel{S4-C2-C2:lem:decomp}{{S4.5.14}{99}{}{theorem.5.14}{}}
\newlabel{S4-C2-C2:sec:abstract}{{S4.5.3}{100}{}{subsection.5.3}{}}
\newlabel{S4-C2-C2:hyp:data}{{S4.5.16}{100}{}{theorem.5.16}{}}
\newlabel{S4-C2-C2:rem:finite}{{S4.5.17}{101}{}{theorem.5.17}{}}
\newlabel{S4-C2-C2:def:seq}{{S4.5.18}{101}{}{theorem.5.18}{}}
\newlabel{S4-C2-C2:lem:consist}{{S4.5.19}{101}{}{theorem.5.19}{}}
\newlabel{S4-C2-C2:def:kappa}{{S4.5.20}{102}{}{theorem.5.20}{}}
\newlabel{S4-C2-C2:lem:ktilde}{{S4.5.21}{102}{}{theorem.5.21}{}}
\newlabel{S4-C2-C2:eq:ktilde}{{S4.5.13}{102}{}{equation.5.13}{}}
\newlabel{S4-C2-C2:lem:kappaprops}{{S4.5.22}{103}{}{theorem.5.22}{}}
\newlabel{S4-C2-C2:rem:change5}{{S4.5.23}{103}{}{theorem.5.23}{}}
\newlabel{S4-C2-C2:lem:locality}{{S4.5.24}{104}{}{theorem.5.24}{}}
\newlabel{S4-C2-C2:def:activity}{{S4.5.25}{104}{}{theorem.5.25}{}}
\newlabel{S4-C2-C2:lem:admissible}{{S4.5.26}{105}{}{theorem.5.26}{}}
\newlabel{S4-C2-C2:lem:E1}{{S4.5.27}{105}{}{theorem.5.27}{}}
\newlabel{S4-C2-C2:eq:E6}{{S4.5.14}{105}{}{equation.5.14}{}}
\newlabel{S4-C2-C2:thm:abstract}{{S4.5.28}{106}{}{theorem.5.28}{}}
\newlabel{S4-C2-C2:eq:E23}{{S4.5.15}{106}{}{equation.5.15}{}}
\newlabel{S4-C2-C2:rem:GMform}{{S4.5.29}{107}{}{theorem.5.29}{}}
\newlabel{S4-C2-C2:rem:six}{{S4.5.30}{107}{}{theorem.5.30}{}}
\newlabel{S4-C2-C2:sec:verify}{{S4.5.4}{107}{}{subsection.5.4}{}}
\newlabel{S4-C2-C2:ssec:data}{{S4.5.4.1}{108}{}{subsubsection.5.4.1}{}}
\newlabel{S4-C2-C2:lem:moments}{{S4.5.31}{108}{}{theorem.5.31}{}}
\newlabel{S4-C2-C2:lem:D3}{{S4.5.32}{109}{}{theorem.5.32}{}}
\newlabel{S4-C2-C2:lem:D4}{{S4.5.33}{110}{}{theorem.5.33}{}}
\newlabel{S4-C2-C2:eq:poinc}{{S4.5.16}{110}{}{equation.5.16}{}}
\newlabel{S4-C2-C2:eq:margin-constants}{{S4.5.17}{110}{}{equation.5.17}{}}
\newlabel{S4-C2-C2:eq:M}{{S4.5.18}{110}{}{equation.5.18}{}}
\newlabel{S4-C2-C2:lem:margin}{{S4.5.34}{110}{}{theorem.5.34}{}}
\newlabel{S4-C2-C2:lem:growth}{{S4.5.35}{111}{}{theorem.5.35}{}}
\newlabel{S4-C2-C2:prop:725}{{S4.5.36}{112}{}{theorem.5.36}{}}
\newlabel{S4-C2-C2:sec:table}{{S4.5.5}{112}{}{subsection.5.5}{}}
\newlabel{S4-S:S4.6}{{S4.6}{113}{}{section.6}{}}
\newlabel{S4-C3-sec:gauss}{{S4.6.1}{113}{}{subsection.6.1}{}}
\newlabel{S4-C3-lem:G1}{{S4.6.1}{114}{}{theorem.6.1}{}}
\newlabel{S4-C3-lem:G2}{{S4.6.2}{114}{}{theorem.6.2}{}}
\newlabel{S4-C3-eq:G2}{{S4.6.1}{114}{}{equation.6.1}{}}
\newlabel{S4-C3-lem:G3}{{S4.6.3}{115}{}{theorem.6.3}{}}
\newlabel{S4-C3-rem:A312}{{S4.6.4}{115}{}{theorem.6.4}{}}
\newlabel{S4-C3-lem:G4}{{S4.6.5}{115}{}{theorem.6.5}{}}
\newlabel{S4-C3-lem:G5}{{S4.6.6}{115}{}{theorem.6.6}{}}
\newlabel{S4-C3-lem:G6}{{S4.6.7}{116}{}{theorem.6.7}{}}
\newlabel{S4-C3-lem:G7}{{S4.6.8}{116}{}{theorem.6.8}{}}
\newlabel{S4-C3-lem:G8}{{S4.6.10}{116}{}{theorem.6.10}{}}
\newlabel{S4-C3b-sec:L729}{{S4.6.2}{116}{}{subsection.6.2}{}}
\newlabel{S4-C3b-eq:split}{{S4.6.2}{117}{}{equation.6.2}{}}
\newlabel{S4-C3b-lem:L729}{{S4.6.11}{117}{}{theorem.6.11}{}}
\newlabel{S4-C3b-lem:mom}{{S4.6.12}{117}{}{theorem.6.12}{}}
\newlabel{S4-C3b-eq:Cstar}{{S4.6.3}{117}{}{equation.6.3}{}}
\newlabel{S4-C3b-rem:L729f}{{S4.6.13}{119}{}{theorem.6.13}{}}
\newlabel{S4-C3b-sec:L730}{{S4.6.3}{119}{}{subsection.6.3}{}}
\newlabel{S4-C3b-lem:L730}{{S4.6.14}{119}{}{theorem.6.14}{}}
\newlabel{S4-C3-sec:L733}{{S4.6.4}{120}{}{subsection.6.4}{}}
\newlabel{S4-C3-eq:Rhat}{{S4.6.4}{120}{}{equation.6.4}{}}
\newlabel{S4-C3-eq:Crho}{{S4.6.5}{121}{}{equation.6.5}{}}
\newlabel{S4-C3-eq:Hkappa}{{S4.6.6}{121}{}{equation.6.6}{}}
\newlabel{S4-C3-lem:rhat}{{S4.6.16}{121}{}{theorem.6.16}{}}
\newlabel{S4-C3-lem:L733}{{S4.6.17}{121}{}{theorem.6.17}{}}
\newlabel{S4-C3-eq:L733}{{S4.6.7}{121}{}{equation.6.7}{}}
\newlabel{S4-C3-eq:L733r}{{S4.6.8}{121}{}{equation.6.8}{}}
\newlabel{S4-C3-eq:II/III}{{S4.6.9}{122}{}{equation.6.9}{}}
\newlabel{S4-C3-eq:R1}{{S4.6.10}{122}{}{equation.6.10}{}}
\newlabel{S4-C3-eq:S2}{{S4.6.11}{123}{}{equation.6.11}{}}
\newlabel{S4-C3-rem:L733changes}{{S4.6.18}{123}{}{theorem.6.18}{}}
\newlabel{S4-C3b-sec:L732}{{S4.6.5}{124}{}{subsection.6.5}{}}
\newlabel{S4-C3b-lem:L732a}{{S4.6.19}{124}{}{theorem.6.19}{}}
\newlabel{S4-C3b-eq:primitive}{{S4.6.12}{124}{}{equation.6.12}{}}
\newlabel{S4-C3b-lem:wwY}{{S4.6.20}{124}{}{theorem.6.20}{}}
\newlabel{S4-C3b-lem:far}{{S4.6.21}{125}{}{theorem.6.21}{}}
\newlabel{S4-C3b-lem:L732b}{{S4.6.22}{125}{}{theorem.6.22}{}}
\newlabel{S4-C3b-lem:L732c}{{S4.6.23}{126}{}{theorem.6.23}{}}
\newlabel{S4-C3b-eq:countN}{{S4.6.13}{126}{}{equation.6.13}{}}
\newlabel{S4-C3-sec:L735}{{S4.6.6}{127}{}{subsection.6.6}{}}
\newlabel{S4-C3-eq:fnn}{{S4.6.14}{127}{}{equation.6.14}{}}
\newlabel{S4-C3-lem:L735}{{S4.6.25}{127}{}{theorem.6.25}{}}
\newlabel{S4-C3-ssec:step1}{{S4.6.6.1}{128}{}{subsubsection.6.6.1}{}}
\newlabel{S4-C3-lem:untr}{{S4.6.26}{128}{}{theorem.6.26}{}}
\newlabel{S4-C3-eq:untr}{{S4.6.15}{128}{}{equation.6.15}{}}
\newlabel{S4-C3-eq:Qexp}{{S4.6.16}{128}{}{equation.6.16}{}}
\newlabel{S4-C3-ssec:step2}{{S4.6.6.2}{128}{}{subsubsection.6.6.2}{}}
\newlabel{S4-C3-lem:JY}{{S4.6.27}{128}{}{theorem.6.27}{}}
\newlabel{S4-C3-rem:n-additivity}{{S4.6.28}{129}{}{theorem.6.28}{}}
\newlabel{S4-C3-ssec:step3}{{S4.6.6.3}{129}{}{subsubsection.6.6.3}{}}
\newlabel{S4-C3-ssec:step4}{{S4.6.6.4}{131}{}{subsubsection.6.6.4}{}}
\newlabel{S4-C3-sec:L736}{{S4.6.7}{131}{}{subsection.6.7}{}}
\newlabel{S4-C3-lem:L736}{{S4.6.30}{131}{}{theorem.6.30}{}}
\newlabel{S4-C3-lem:pointwise736}{{S4.6.31}{132}{}{theorem.6.31}{}}
\newlabel{S4-C3-eq:T4pointwise}{{S4.6.17}{132}{}{equation.6.17}{}}
\newlabel{S4-C3-sec:P737}{{S4.6.8}{133}{}{subsection.6.8}{}}
\newlabel{S4-C3-prop:P737}{{S4.6.33}{133}{}{theorem.6.33}{}}
\newlabel{S4-C3-eq:Astar}{{S4.6.18}{135}{}{equation.6.18}{}}
\newlabel{S4-C3-lem:cellcount}{{S4.6.34}{135}{}{theorem.6.34}{}}
\newlabel{S4-C3-lem:wick}{{S4.6.35}{135}{}{theorem.6.35}{}}
\newlabel{S4-C3-sec:P738}{{S4.6.9}{136}{}{subsection.6.9}{}}
\newlabel{S4-C3-lem:rates}{{S4.6.37}{136}{}{theorem.6.37}{}}
\newlabel{S4-C3-prop:P738}{{S4.6.38}{139}{}{theorem.6.38}{}}
\newlabel{S4-C3-eq:margins}{{S4.6.19}{139}{}{equation.6.19}{}}
\newlabel{S4-C3b-sec:L738}{{S4.6.10}{140}{}{subsection.6.10}{}}
\newlabel{S4-C3b-cor:inB7}{{S4.6.40}{140}{}{theorem.6.40}{}}
\newlabel{S4-C3b-lem:L738}{{S4.6.41}{141}{}{theorem.6.41}{}}
\newlabel{S4-C3b-prop:P739}{{S4.6.42}{141}{}{theorem.6.42}{}}
\newlabel{S4-C3b-thm:T740}{{S4.6.43}{142}{}{theorem.6.43}{}}
\newlabel{S4-C3b-lem:L741}{{S4.6.44}{142}{}{theorem.6.44}{}}
\newlabel{S4-C3b-cor:consts}{{S4.6.45}{143}{}{theorem.6.45}{}}
\newlabel{S4-S:S4.7}{{S4.7}{144}{}{section.7}{}}
\newlabel{S4-C3b-sec:B1}{{S4.7.1}{144}{}{subsection.7.1}{}}
\newlabel{S4-C3b-ssec:B-setting}{{S4.7.1.1}{144}{}{subsubsection.7.1.1}{}}
\newlabel{S4-C3b-eq:G2cell}{{S4.7.1}{144}{}{equation.7.1}{}}
\newlabel{S4-C3b-ssec:B1}{{S4.7.1.2}{145}{}{subsubsection.7.1.2}{}}
\newlabel{S4-C3b-lem:B1}{{S4.7.1}{145}{}{theorem.7.1}{}}
\newlabel{S4-C3b-sec:B2}{{S4.7.1.3}{146}{}{subsubsection.7.1.3}{}}
\newlabel{S4-C3b-lem:B2}{{S4.7.3}{146}{}{theorem.7.3}{}}
\newlabel{S4-C3b-ssec:B3}{{S4.7.1.4}{147}{}{subsubsection.7.1.4}{}}
\newlabel{S4-C3b-lem:B3}{{S4.7.4}{147}{}{theorem.7.4}{}}
\newlabel{S4-C3b-sec:B4}{{S4.7.2}{148}{}{subsection.7.2}{}}
\newlabel{S4-C3b-lem:growth}{{S4.7.5}{148}{}{theorem.7.5}{}}
\newlabel{S4-C3b-lem:B4}{{S4.7.6}{148}{}{theorem.7.6}{}}
\newlabel{S4-C3b-sec:B5}{{S4.7.2.2}{149}{}{subsubsection.7.2.2}{}}
\newlabel{S4-C3b-lem:B5}{{S4.7.7}{150}{}{theorem.7.7}{}}
\newlabel{S4-C3b-ssec:B6}{{S4.7.2.3}{151}{}{subsubsection.7.2.3}{}}
\newlabel{S4-C3b-thm:B6}{{S4.7.8}{151}{}{theorem.7.8}{}}
\newlabel{S4-C3b-lem:nj}{{S4.7.9}{152}{}{theorem.7.9}{}}
\newlabel{S4-C3b-sec:B7}{{S4.7.3}{152}{}{subsection.7.3}{}}
\newlabel{S4-C3b-lem:B8}{{S4.7.10}{152}{}{theorem.7.10}{}}
\newlabel{S4-C3b-lem:B9}{{S4.7.11}{153}{}{theorem.7.11}{}}
\newlabel{S4-C3b-prop:B10}{{S4.7.12}{153}{}{theorem.7.12}{}}
\newlabel{S4-C3b-prop:B7}{{S4.7.13}{154}{}{theorem.7.13}{}}
\newlabel{S4-C3b-eq:B7}{{S4.7.2}{154}{}{equation.7.2}{}}
\newlabel{S4-C3b-rem:B11}{{S4.7.14}{156}{}{theorem.7.14}{}}
\newlabel{S4-S:S4.8}{{S4.8}{156}{}{section.8}{}}
\newlabel{S4-C3b-sec:primadm}{{S4.8.1}{156}{}{subsection.8.1}{}}
\newlabel{S4-C3b-prop:primadm}{{S4.8.1}{156}{}{theorem.8.1}{}}
\newlabel{S4-C4-s:trees}{{S4.8.2}{156}{}{subsection.8.2}{}}
\newlabel{S4-C4-def:theta}{{S4.8.2}{157}{}{theorem.8.2}{}}
\newlabel{S4-C4-eq:Ky-theta}{{S4.8.1}{157}{}{equation.8.1}{}}
\newlabel{S4-C4-def:treeoftheta}{{S4.8.3}{157}{}{theorem.8.3}{}}
\newlabel{S4-C4-lem:A1}{{S4.8.4}{157}{}{theorem.8.4}{}}
\newlabel{S4-C4-eq:treeform}{{S4.8.2}{157}{}{equation.8.2}{}}
\newlabel{S4-C4-rem:A1changes}{{S4.8.5}{158}{}{theorem.8.5}{}}
\newlabel{S4-C4-def:linkdatum}{{S4.8.6}{158}{}{theorem.8.6}{}}
\newlabel{S4-C4-def:kappaprime}{{S4.8.7}{159}{}{theorem.8.7}{}}
\newlabel{S4-C4-eq:kappaprime}{{S4.8.3}{159}{}{equation.8.3}{}}
\newlabel{S4-C4-lem:treesum}{{S4.8.8}{159}{}{theorem.8.8}{}}
\newlabel{S4-C4-rem:treesum}{{S4.8.9}{159}{}{theorem.8.9}{}}
\newlabel{S4-C4-s:link}{{S4.8.3}{160}{}{subsection.8.3}{}}
\newlabel{S4-C4-lem:elconn}{{S4.8.10}{160}{}{theorem.8.10}{}}
\newlabel{S4-C4-lem:rooting}{{S4.8.11}{160}{}{theorem.8.11}{}}
\newlabel{S4-C4-def:Ld}{{S4.8.12}{160}{}{theorem.8.12}{}}
\newlabel{S4-C4-lem:L0Ld}{{S4.8.13}{160}{}{theorem.8.13}{}}
\newlabel{S4-C4-lem:growth}{{S4.8.14}{161}{}{theorem.8.14}{}}
\newlabel{S4-C4-lem:MSTcount}{{S4.8.15}{161}{}{theorem.8.15}{}}
\newlabel{S4-C4-def:phi}{{S4.8.16}{161}{}{theorem.8.16}{}}
\newlabel{S4-C4-lem:A7}{{S4.8.17}{161}{}{theorem.8.17}{}}
\newlabel{S4-C4-rem:A7src}{{S4.8.18}{162}{}{theorem.8.18}{}}
\newlabel{S4-C4-s:A8}{{S4.8.4}{162}{}{subsection.8.4}{}}
\newlabel{S4-C4-lem:entropy}{{S4.8.19}{162}{}{theorem.8.19}{}}
\newlabel{S4-C4-prop:A8}{{S4.8.20}{163}{}{theorem.8.20}{}}
\newlabel{S4-C4-rem:A8changes}{{S4.8.21}{164}{}{theorem.8.21}{}}
\newlabel{S4-C4-s:core}{{S4.8.5}{164}{}{subsection.8.5}{}}
\newlabel{S4-C4-def:seedconsts}{{S4.8.22}{164}{}{theorem.8.22}{}}
\newlabel{S4-C4-lem:MSigma}{{S4.8.23}{165}{}{theorem.8.23}{}}
\newlabel{S4-C4-prop:A9}{{S4.8.24}{165}{}{theorem.8.24}{}}
\newlabel{S4-C4-eq:core}{{S4.8.4}{165}{}{equation.8.4}{}}
\newlabel{S4-C4-rem:ledger}{{S4.8.25}{166}{}{theorem.8.25}{}}
\newlabel{S4-C4-lem:split}{{S4.8.26}{166}{}{theorem.8.26}{}}
\newlabel{S4-C4-lem:polygeom}{{S4.8.27}{166}{}{theorem.8.27}{}}
\newlabel{S4-C4-lem:753}{{S4.8.28}{167}{}{theorem.8.28}{}}
\newlabel{S4-C4-s:77}{{S4.8.6}{168}{}{subsection.8.6}{}}
\newlabel{S4-C4-lem:744}{{S4.8.29}{168}{}{theorem.8.29}{}}
\newlabel{S4-C4-lem:746}{{S4.8.30}{168}{}{theorem.8.30}{}}
\newlabel{S4-C4-lem:747}{{S4.8.31}{169}{}{theorem.8.31}{}}
\newlabel{S4-C4-lem:prim}{{S4.8.32}{169}{}{theorem.8.32}{}}
\newlabel{S4-C4-lem:prim1}{{S4.8.33}{170}{}{theorem.8.33}{}}
\newlabel{S4-C4-cor:long}{{S4.8.34}{170}{}{theorem.8.34}{}}
\newlabel{S4-C4-prop:751}{{S4.8.35}{170}{}{theorem.8.35}{}}
\newlabel{S4-C4-thm:752}{{S4.8.36}{171}{}{theorem.8.36}{}}
\newlabel{S4-C4-eq:KSr}{{S4.8.5}{171}{}{equation.8.5}{}}
\newlabel{S4-C4-s:78}{{S4.8.7}{172}{}{subsection.8.7}{}}
\newlabel{S4-C4-lem:754}{{S4.8.38}{172}{}{theorem.8.38}{}}
\newlabel{S4-C4-lem:755}{{S4.8.39}{173}{}{theorem.8.39}{}}
\newlabel{S4-C4-eq:NFpieces}{{S4.8.6}{174}{}{equation.8.6}{}}
\newlabel{S4-C4-prop:756}{{S4.8.40}{174}{}{theorem.8.40}{}}
\newlabel{S4-C4-prop:757}{{S4.8.42}{175}{}{theorem.8.42}{}}
\newlabel{S4-C4-lem:758}{{S4.8.43}{175}{}{theorem.8.43}{}}
\newlabel{S4-C4-s:79}{{S4.8.8}{176}{}{subsection.8.8}{}}
\newlabel{S4-C4-lem:759}{{S4.8.44}{176}{}{theorem.8.44}{}}
\newlabel{S4-C4-lem:760}{{S4.8.45}{176}{}{theorem.8.45}{}}
\newlabel{S4-C4-thm:761}{{S4.8.46}{176}{}{theorem.8.46}{}}
\newlabel{S4-C4-eq:bbeta}{{S4.8.7}{177}{}{equation.8.7}{}}
\newlabel{S4-C4-rem:762}{{S4.8.47}{177}{}{theorem.8.47}{}}
\newlabel{S4-C4-lem:A11}{{S4.8.48}{177}{}{theorem.8.48}{}}
\newlabel{S4-C4-s:sources}{{S4.8.9}{178}{}{subsection.8.9}{}}
\newlabel{S4-C4-ss:B78}{{S4.8.9.2}{178}{}{subsubsection.8.9.2}{}}
\newlabel{S4-S:S4.9}{{S4.9}{179}{}{section.9}{}}
\newlabel{S4-S9-s:gineq}{{S4.9.1}{179}{}{subsection.9.1}{}}
\newlabel{S4-S9-lem:twoweight}{{S4.9.1}{179}{}{theorem.9.1}{}}
\newlabel{S4-S9-lem:wilsonpair}{{S4.9.2}{180}{}{theorem.9.2}{}}
\newlabel{S4-S9-cor:ginibre}{{S4.9.3}{180}{}{theorem.9.3}{}}
\newlabel{S4-S9-rem:mmsp}{{S4.9.4}{180}{}{theorem.9.4}{}}
\newlabel{S4-S9-s:91}{{S4.9.2}{180}{}{subsection.9.2}{}}
\newlabel{S4-S9-prop:91}{{S4.9.5}{180}{}{theorem.9.5}{}}
\newlabel{S4-S9-s:92}{{S4.9.3}{181}{}{subsection.9.3}{}}
\newlabel{S4-S9-cor:92}{{S4.9.7}{181}{}{theorem.9.7}{}}
\newlabel{S4-S9-s:GG}{{S4.9.4}{182}{}{subsection.9.4}{}}
\newlabel{S4-S9-lem:ugauge}{{S4.9.9}{182}{}{theorem.9.9}{}}
\newlabel{S4-S9-lem:hop}{{S4.9.10}{182}{}{theorem.9.10}{}}
\newlabel{S4-S9-thm:conc}{{S4.9.11}{183}{}{theorem.9.11}{}}
\newlabel{S4-S9-prop:93}{{S4.9.12}{184}{}{theorem.9.12}{}}
\newlabel{S4-S9-s:94}{{S4.9.5}{184}{}{subsection.9.5}{}}
\newlabel{S4-S9-cor:94}{{S4.9.13}{184}{}{theorem.9.13}{}}
\newlabel{S4-S9-s:95}{{S4.9.6}{184}{}{subsection.9.6}{}}
\makeatother

